Federated Distillation based Indoor Localization for IoT Networks

Federated distillation (FD) paradigm has been recently proposed as a promising alternative to federated learning (FL) especially in wireless sensor networks with limited communication resources. However, all state-of-the art FD algorithms are designed for only classification tasks and less attention has been given to regression tasks. In this work, we propose an FD framework that properly operates on regression learning problems. Afterwards, we present a use-case implementation by proposing an indoor localization system that shows a good trade-off communication load vs. accuracy compared to federated learning (FL) based indoor localization. With our proposed framework, we reduce the number of transmitted bits by up to 98%. Moreover, we show that the proposed framework is much more scalable than FL, thus more likely to cope with the expansion of wireless networks.

==> common/acknowledgments.tex <==
\section*{Acknowledgments}
The acknowledgement goes here.

==> corrections.tex <==
\section{Modifications to make}
\begin{itemize}
    \item Introduce real time locating system (RTLS) since this a rtls problem.
    \item Reduce explanation of FL and FD. the concepts are well established.
    \item More contributions(the contributions are quite incremental compared to existing works on FL/FD.): Label balancing for instance.
   done \item Motivation: Why FL/FD should be deployed in such scenario? What is the benefit?
    \item Considering FL/FD processes, latency (#of rounds) vs accuracy tradeoffs must be considered or better highlithed: for example, how many rounds are required by FL/FD to achieve a same MAE?. FD might save bandwidth on each round, but probably it requires much more rounds than FL to converge (?). 

    
    
\end{itemize}

\section{Problem formulation}
\subsection{Training set-up}: RSSI data from multiple anchor nodes are fused and collected on a server. We substitute this by crowdsourcing, data are no longuer sent to the server. Zoning is performed and crowdsourcing is done in each zone to train a zone level model. 
\subsection{Inference set-up}

==> sections/discussion.tex <==
\section{Discussion and Future works}
\label{sec:discussion}
% The Discussion goes here
% deal with missing segment, GAN 
% Investigate more advanced segmentation strategy
% Proxy data to enhance the model performance
%% Auto-Generate the copy of client data to server.
% Error prediction for  target estimation adjustment
% third segmentation strategy
The work presented in this paper comes to fill a void by setting-up a fresh method to distill knowledge in IoT networks in a federated manner, regarding regression problems. The simulation results and the performance analysis provide the proof of concept of our proposed framework. This framework appears to have a great potential for a large variety of applications such  as localization in IoT networks. \\
Although the performance shown by our framework are satisfactory, it can be further improved by investigating different paths, among others the followings:
\begin{itemize}
    \item \textbf{Unbalanced/Missing Segments:} Similar to the problem of missing labels in classification tasks, after segmentation of target variables, we are more likely to end up with unbalanced and or missing data in local private datasets, accentuating the phenomenon of \ac{N.I.I.D} data whose a proper mitigation method should be proposed. For instance, \acp{GAN} can be introduced in this work to improve the data distributions.
    \item \textbf{Segmentation Strategy:} the performance of a federated learning system greatly relies on the data distribution which is affected by the segmentation strategy in this framework. So investigating a more robust segmentation method can be of a great importance.
   \item \textbf{Proxy data:} In our framework, the knowledge distillation in the network is done that difficult way because of the private aspect of the local data. If a public dataset is available for the given ML problem, then it can leverage a more fluid distillation process, hence enhancing the system performance. Otherwise, we can think of creating fake copies of user data in the server using for instance \acp{GAN}.
   \item \textbf{Error prediction:} Given a segmentation strategy, the predictability of estimation errors can lead to a great enhancement of the system performance by adjusting the estimations accordingly.
   \item \textbf{Model distillation:} We showed that the number of transmitted bits in our framework relies mainly on the number of segments and the number of target variables. With this in mind, we can define different models for FD students according to their capabilities, thus reducing the IoT devices heterogeneity problem.
   \item \textbf{FL/FD mix-up:} In wireless networks, a great asymmetry exits between the uplink and the downlink, and the communication challenge for IoT devices mainly happens on the uplink. This can be exploited so that during the training FD is performed on the uplink to reduce the communication cost and on the less challenging downlink, FL is used. In the other hand,
   an IoT network is more often composed of heterogeneous devices making difficult the adoption a unified learning model. Therefore, we can use FL in both uplink and downlink for high capabilities devices, while keeping full FD for the remaining. 
\end{itemize}
